Gas Excitation in ULIRGS: Maps of Diagnostic Emission-Line Ratios in Space and Velocity

Emission-line spectra extracted at multiple locations across 39 ultraluminous infrared galaxies have been compiled into a spectrophotometric atlas. Line profiles of H alpha, [N II], [S II], [O I], H beta, and [O III] are resolved and fit jointly with common velocity components. Diagnostic ratios of these line fluxes are presented in a series of plots, showing how the Doppler shift, line width, gas excitation, and surface brightness change with velocity at fixed position and also with distance from the nucleus. One general characteristic of these spectra is the presence of shocked gas extending many kiloparsecs from the nucleus. In some systems, the shocked gas appears as part of a galactic gas disk based on its rotation curve. These gas disks appear primarily during the early stages of the merger. The general characteristics of the integrated spectra are also presented.

==> i15245_bbc.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    15245    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering
\epsfig{file=i15245pos3.eps, keepaspectratio=true, width=\linewidth}
\epsfig{file=i15245.eps, keepaspectratio=true, width=\linewidth}
\caption{\label{fig:i15245_bbc}
}
\end{figure}
\clearpage



==> i15245_prof.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   15245     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering
\epsfig{file=i15245_nest_grid_res.eps, keepaspectratio=true, width=0.9\linewidth}
\caption{\label{fig:i15245_prof}
}
\end{figure}
\clearpage



